MIC: Mining Interclass Characteristics for Improved Metric Learning

Metric learning seeks to embed images of objects suchthat class-defined relations are captured by the embeddingspace. However, variability in images is not just due to different depicted object classes, but also depends on other latent characteristics such as viewpoint or illumination. In addition to these structured properties, random noise further obstructs the visual relations of interest. The common approach to metric learning is to enforce a representation that is invariant under all factors but the ones of interest. In contrast, we propose to explicitly learn the latent characteristics that are shared by and go across object classes. We can then directly explain away structured visual variability, rather than assuming it to be unknown random noise. We propose a novel surrogate task to learn visual characteristics shared across classes with a separate encoder. This encoder is trained jointly with the encoder for class information by reducing their mutual information. On five standard image retrieval benchmarks the approach significantly improves upon the state-of-the-art.

==> tables/architectures.tex <==

\begin{table}
\begin{center}
\begin{tabular}{l|c|c|ccc}
\hline
Method & Network & Dim & CARS196 & CUB200 & SOP \\
\hline\hline
SemiHard & Iv3 & 64 & - & - & - \\
SemiHard & RN50 & 128 & 71.3 & 58.9 & 69.8 \\
SemiHard & RN50 & 512 & 74.5 & 62.6 & 69.9 \\
\hline\hline
Margin & Iv3 & 64 & - & - & - \\
Margin & RN50 & 128 & 75.0 & 61.4 & 70.3 \\
Margin & RN50 & 512 & - & - & - \\
\hline
HIP & Iv3 & 64 & - & - & - \\
HIP & RN50 & 128 & 78.0 & 62.2 & 73.0 \\
HIP & RN50 & 512 & - & - & - \\
\hline
\end{tabular}
\end{center}
\caption{Different architectures and embedding dimensions.RN50: ResNet50, Iv3: InceptionV3. All implementations are our own}
\label{tab:architectures}
\end{table}



% \begin{table}
% \begin{center}
% \begin{tabular}{l|c|c|c|c|c|c|c}
% \hline
% \#Clusters & 5 & 10 & 20& 30 & 40 & 50 & 80\\
% \hline\hline
% CARS196 & 0.784 & 0.787 & 0.792 & \textbf{0.797} & 0.794 & 0.795 & 0.786\\
% CUB200  & 0.594 & 0.597 & 0.611 & 0.614 & \textbf{0.628} & 0.626 & 0.627\\
% SOP     & - & - & - & - & - & - & -\\
% \hline
% \end{tabular}
% \end{center}
% \label{tab:cluster}
% \caption{Ablation study: influence of the number of clusters for Recall@1. Fixed cluster label update period of 3 was used without higher learning rate and no scheduling.}
% \end{table}



==> tables/tables.tex <==

\begin{table}
\begin{center}
\begin{tabular}{l|c|ccc|c}
\hline
R@k & Dim & 1 & 2 & 4  & NMI \\
\hline
LiftStruct \cite{lifted} & 512 & 48.3 & 61.1 & 71.8 & 55.1 \\
FacilityLoc \cite{facilitylocation} & 64 & 67.0 & 83.7 & 93.2 & - \\
SmartMin \cite{smartmining} & 64 & 64.7 & 76.2 & 84.2 & - \\
N-pairs\cite{npairs} & 64 & 71.1 & 79.7 & 86.5 & - \\
Angular\cite{angular} & 512 & 71.4 & 81.4 & 87.5& - \\
ProxyNCA\cite{proxynca} & 64 & 73.2 & 82.4 & 86.4 & - \\
HDC\cite{hdc} & 384 & 73.7 & 83.2 & 89.5 & - \\
DAML\cite{daml} & 512 & 75.1 & 83.8 & 89.7 & 66.0 \\
HTG\cite{htg} & - & 76.5 & 84.7 & 90.4 & - \\
BIER\cite{bier} & 512 & 78.0 & 85.8 & 91.1& - \\
HTL\cite{htl} & 512 & 81.4 & 88.0 & 92.7.8  & - \\
DVML\cite{dvml} & 512 & 82.0 & 88.4 & 93.3 & 67.6 \\
A-BIER\cite{abier} & 512 & 82.0 & 89.0 & 93.2  & - \\
\hline
DREML\cite{dreml} & 9216 & 86.0 & 91.7 & 95.0 & 76.4 \\
\hline
Semihard\cite{semihard} & - & 51.5 & 63.8 & 73.5 & 53.4 \\
Semihard* & 128 & 71.3 & 80.7 & 87.5 &62.5 \\
\textbf{COD+semih} & 128 & - & - & - & - \\
Margin\cite{margin}     & 128 & 79.6 & 86.5 & 91.9 & 69.0 \\
Margin*                 & 128 & 80.0 & 87.7 & 92.3 & 66.3 \\
\textbf{COD+margin}     & 128 & \textbf{82.4} & 89.2 & 93.4 & \textbf{70.0} \\
\hline
Semihard* & 512 & 75.1 & 83.6 & 89.8 & 62.8\\
\textbf{COD+semih} & 512 & - & - & - & - \\
% \textbf{COD+margin}  & 256 & 81.1 & 88.2 & 92.6 & 96.0 & 68.8 \\
Margin* & 512 & 80.1 & 87.1 & 91.7 & 64.1 \\
\textbf{COD+margin} & 512 & - & - & - & - \\
% \hline\hline
\hline
\end{tabular}
\end{center}
\caption{Recall@k for k nearest neighbor and NMI on CARS196 \cite{cars196}. (*) indicates our best re-implementation with ResNet50.}
\label{tab:cars}
\end{table}


\begin{table}
\begin{center}
\begin{tabular}{l|c|ccc|c}
\hline
R@k & Dim & 1 & 10 & 100 & NMI \\
\hline
Histogram\cite{histogram} & - & 63.9 & 81.7 & 92.2 &  - \\
BinDev\cite{bindeviance} & - & 65.5 & 82.3 & 92.3 &  -\\
LiftStruct \cite{lifted} & 512 & 63.0 & 80.5 & 91.7 & 87.4 \\
FacilityLoc \cite{facilitylocation} & 64 & 67.0 & 83.7 & 93.2 & -  \\
N-pairs\cite{npairs} & 512 & 67.7& 83.8 & 93.0 & 88.1 \\
Angular\cite{angular} & 512 & 70.9 & 85.0 & 93.5 & 88.6 \\
DAML\cite{daml} & 512 & 68.4 & 83.5 & 92.3 & 89.4 \\
HDC\cite{hdc} & 384 & 69.5 & 84.4 & 92.8 & - \\
DVML\cite{dvml} & 512 & 70.2 & 85.2 & 93.8 & \textbf{90.8} \\
BIER\cite{bier} & 512 & 72.7 & 86.5 & 94.0 & - \\
ProxyNCA\cite{proxynca} & 64 & 73.7 & - & - & - \\
A-BIER\cite{abier} & 512 & 74.2 & 86.9 & 94.0 & - \\
HTL\cite{htl} & 512 & 69.5 & 84.4 & 92.8 &  - \\
\hline
Semi-hard\cite{semihard} & - & 66.7 & 82.4 & 91.9 &  89.5 \\
Semihard* & 128 & 67.4 & 83.9 & 92.3 & 88.5 \\
\textbf{COD+semih} & 128 & - & - & - & - \\
Margin\cite{margin}     & 128 & 72.7 & 86.2 & 93.8 & \textbf{90.7} \\
Margin*                 & 128 & 73.0 & 85.9 & 93.3 & 89.3 \\
\textbf{COD+margin}     & 128 & \textbf{75.2} & 86.8 & 93.9 &  \textbf{90.6} \\
\hline
Semihard* & 512 & 70.1 & 85.7 & 92.7 & 88.6 \\
\textbf{COD+semih} & 512 & - & - & - & - \\
% \textbf{COD+margin}  & 256 & - & - & - &  - \\
Margin*                 & 512 & 73.3 & 87.8 & 95.1 & \textbf{91.0} \\
\textbf{COD+margin}     & 512 & - & - & - &  - \\
\hline
\end{tabular}
\end{center}
\caption{Recall@k for k nearest neighbor and NMI on Stanford Online Products \cite{lifted}. (*) indicates our best re-implementation with ResNet50}
\label{tab:sop}
\end{table}

\begin{table}
\begin{center}
\begin{tabular}{l|c|ccc|c}
\hline
R@k & Dim & 1 & 2 & 4 &  NMI \\
\hline
LiftStruct \cite{lifted} & 512 & 46.6 & 58.1 & 69.8 & 56.2 \\
FacilityLoc \cite{facilitylocation} & 64 & 48.2 & 61.4 & 71.8 & 59.2 \\
SmartMin \cite{smartmining} & 64 & 49.8 & 62.3 & 74.1 & - \\
ProxyNCA\cite{proxynca} & 64 & 49.2 & 61.9 & 67.9 & 64.9 \\
Histogram\cite{histogram} & & 50.3 & 61.9 & 72.6  & - \\
BinDev\cite{bindeviance} & - & 52.8 & 64.4 & 74.7  & - \\
N-pairs\cite{npairs} & 64 & 51.0 & 63.3 & 74.3 &  60.4 \\
DVML\cite{dvml} & 512 & 52.7 & 65.1 & 75.5 &61.4 \\
DAML\cite{daml} & 512 & 52.7 & 65.4 & 75.5 & 61.3 \\
Angular\cite{angular} & 512 & 54.7 & 66.3 & 76.0& 61.1 \\
HDC\cite{hdc} & 384 & 53.6 & 65.7 & 77.0 & - \\
BIER\cite{bier} & 512 & 55.3 & 67.2 & 76.9 & - \\
HTL\cite{htl} & 512 & 57.1 & 68.8 & 78.7 & - \\
A-BIER\cite{abier} & 512 & 57.5 & 68.7 & 78.3& - \\
HTG\cite{htg} & - & 59.5 & 71.8 & 81.3 & - \\
\hline
DREML\cite{dreml} & 9216 & 63.9 & 75.0 & 83.1 &  67.8 \\
\hline
Semihard\cite{semihard} & - & 42.6 & 55.0 & 66.4 & 55.4 \\
Semihard* & 128 & 56.8 & 69.1 & 79.8.7 & 63.0 \\
\textbf{COD+semih} & 128 & - & - & - &- \\
Margin\cite{margin}     & 128 & 63.6 & 74.4 & 83.1 &69.0 \\
Margin*                 & 128 & 62.9 & 74.1 & 82.9 &  66.3 \\
\textbf{COD+margin}     & 128 & \textbf{66.6} & 76.5 & 84.8& \textbf{69.0} \\
\hline
Semihard* & 512 & 60.6 & 72.3 & 82.3 &  64.5 \\
\textbf{COD+semih} & 512 & - & - & - & - \\
% \textbf{COD+margin}  & 256 & - & - & - & - & - \\
Margin* & 512 & 65.1 & 75.6 & 84.2 &  67.2 \\
\textbf{COD+margin} & 512 & - & - & -  & - \\
% \hline\hline
\hline
\end{tabular}
\end{center}
\caption{Recall@k for k nearest neighbor and NMI on CUB200-2011 \cite{cub200-2011}. (*) indicates our best re-implementation with ResNet50.}
\label{tab:cub}
\end{table}



\begin{table}
\begin{center}
\begin{tabular}{l|c|c|ccc}
\hline
Method & Network & Dim & CARS196 & CUB200 & SOP \\
\hline\hline
SemiHard & Iv3 & 64 & - & - & - \\
SemiHard & RN50 & 128 & 71.3 & 58.9 & 69.8 \\
SemiHard & RN50 & 512 & 74.5 & 62.6 & 69.9 \\
\hline\hline
Margin & Iv3 & 64 & - & - & - \\
Margin & RN50 & 128 & 75.0 & 61.4 & 70.3 \\
Margin & RN50 & 512 & - & - & - \\
\hline
COD & Iv3 & 64 & - & - & - \\
COD & RN50 & 128 & 78.0 & 62.2 & 73.0 \\
COD & RN50 & 512 & - & - & - \\
\hline
\end{tabular}
\end{center}
\caption{Different architectures and embedding dimensions.RN50: ResNet50, Iv3: InceptionV3. All implementations are our own}
\label{tab:architectures}
\end{table}












% \begin{table}
% \begin{center}
% \begin{tabular}{l|c|cccc|c}
% \hline
% R@k & Dim & 1 & 2 & 4 & 8 & NMI \\
% \hline
% LiftStruct \cite{lifted} & 512 & 48.3 & 61.1 & 71.8 & 81.1 & 55.1 \\
% FacilityLoc \cite{facilitylocation} & 64 & 67.0 & 83.7 & 93.2 & - & - \\
% SmartMin \cite{smartmining} & 64 & 64.7 & 76.2 & 84.2 & 90.2 & - \\
% N-pairs\cite{npairs} & 64 & 71.1 & 79.7 & 86.5 & 91.6 & - \\
% Angular\cite{angular} & 512 & 71.4 & 81.4 & 87.5 & 92.1 & - \\
% ProxyNCA\cite{proxynca} & 64 & 73.2 & 82.4 & 86.4 & 87.8 & - \\
% HDC\cite{hdc} & 384 & 73.7 & 83.2 & 89.5 & 93.8 & - \\
% DAML\cite{daml} & 512 & 75.1 & 83.8 & 89.7 & 93.5 & 66.0 \\
% HTG\cite{htg} & - & 76.5 & 84.7 & 90.4 & 94.0 & - \\
% BIER\cite{bier} & 512 & 78.0 & 85.8 & 91.1 & 95.1 & - \\
% HTL\cite{htl} & 512 & 81.4 & 88.0 & 92.7.8 & 95.7 & - \\
% DVML\cite{dvml} & 512 & 82.0 & 88.4 & 93.3 & 96.3 & 67.6 \\
% A-BIER\cite{abier} & 512 & 82.0 & 89.0 & 93.2 & 96.1 & - \\
% \hline
% DREML\cite{dreml} & 9216 & 86.0 & 91.7 & 95.0 & 97.2 & 76.4 \\
% \hline
% Semihard\cite{semihard} & - & 51.5 & 63.8 & 73.5 & 82.4 & 53.4 \\
% Semihard* & 128 & 71.3 & 80.7 & 87.5 & 93.0 & 62.5 \\
% \textbf{COD+semih} & 128 & - & - & - & - & - \\
% Margin\cite{margin}     & 128 & 79.6 & 86.5 & 91.9 & 95.1 & 69.0 \\
% Margin*                 & 128 & 80.0 & 87.7 & 92.3 & 95.5 & 66.3 \\
% \textbf{COD+margin}     & 128 & \textbf{82.4} & 89.2 & 93.4 & 96.2 & \textbf{70.0} \\
% \hline
% Semihard* & 512 & 75.1 & 83.6 & 89.8 & 94.1 & 62.8\\
% \textbf{COD+semih} & 512 & - & - & - & - & - \\
% % \textbf{COD+margin}  & 256 & 81.1 & 88.2 & 92.6 & 96.0 & 68.8 \\
% Margin* & 512 & 80.1 & 87.1 & 91.7 & 94.8 & 64.1 \\
% \textbf{COD+margin} & 512 & - & - & - & - & - \\
% % \hline\hline
% \hline
% \end{tabular}
% \end{center}
% \label{tab:cars}
% \caption{Recall@k for k nearest neighbor and NMI on CARS196 \cite{cars196}. (*) indicates our best re-implementation with ResNet50.}
% \end{table}


% \begin{table}
% \begin{center}
% \begin{tabular}{lcccccc}
% \hline
% R@k & Dim & 1 & 10 & 100 & 1000 & NMI \\
% \hline
% Histogram\cite{histogram} & & 63.9 & 81.7 & 92.2 & 97.7 & - \\
% Binomial Deviance\cite{binomial} & & 65.5 & 82.3 & 92.3 & 97.6 & -\\
% Triplet Semi-hard\cite{semihard} & & 66.7 & 82.4 & 91.9 & - & 89.5 \\
% LiftedStruct \cite{lifted} & & 63.0 & 80.5 & 91.7 & 97.5 & 87.4 \\
% FacilityLoc \cite{floc} & & 67.0 & 83.7 & 93.2 & - & - \\
% N-pairs\cite{npairs} & & 67.7& 83.8 & 93.0 & 97.8 & 88.1 \\
% Angular\cite{angular} & & 70.9 & 85.0 & 93.5 & 98.0 & 88.6 \\
% DAML\cite{daml} & & 68.4 & 83.5 & 92.3 & - & 89.4 \\
% HDC\cite{hdc} & & 69.5 & 84.4 & 92.8 & 97.7 & - \\
% DVML\cite{dvml} & & 70.2 & 85.2 & 93.8 & - & \textbf{90.8} \\
% BIER\cite{bier} & 512 & 72.7 & 86.5 & 94.0 & 98.0 & - \\
% ProxyNCA\cite{proxynca} & & 73.7 & - & - & - & - \\
% A-BIER\cite{abier} & 512 & \textbf{74.2} & \textbf{86.9} & 94.0 & 98.0 & - \\
% HTL\cite{htl} & 512 & 69.5 & 84.4 & 92.8 & 97.7 & - \\
% Margin\cite{margin} & 128 & 72.7 & 86.2 & 93.8 & 98.0 & \textbf{90.7} \\
% OUR Margin baseline* & 128 & 70.3 & - & - & - & 89.3 \\
% \textbf{COD (our)} & 128 & 73.0 & - & - & - & \textbf{89.4} \\
% \hline
% \end{tabular}
% \end{center}
% \caption{Recall@k for k nearest neighbor and NMI on Stanford Online Products \cite{sop}}
% \end{table}



% \begin{table}
% \begin{center}
% \begin{tabular}{l|c|cccc|c}
% \hline
% R@k & Dim & 1 & 2 & 4 & 8 & NMI \\
% \hline
% LiftStruct \cite{lifted} & 512 & 46.6 & 58.1 & 69.8 & 80.2 & 56.2 \\
% FacilityLoc \cite{facilitylocation} & 64 & 48.2 & 61.4 & 71.8 & 81.9 & 59.2 \\
% SmartMin \cite{smartmining} & 64 & 49.8 & 62.3 & 74.1 & 83.3 & - \\
% ProxyNCA\cite{proxynca} & 64 & 49.2 & 61.9 & 67.9 & 72.4 & 64.9 \\
% Histogram\cite{histogram} & & 50.3 & 61.9 & 72.6 & 82.4 & - \\
% BinDev\cite{bindeviance} & - & 52.8 & 64.4 & 74.7 & 83.9 & - \\
% N-pairs\cite{npairs} & 64 & 51.0 & 63.3 & 74.3 & 83.2 & 60.4 \\
% DVML\cite{dvml} & 512 & 52.7 & 65.1 & 75.5 & 84.3 & 61.4 \\
% DAML\cite{daml} & 512 & 52.7 & 65.4 & 75.5 & 84.3 & 61.3 \\
% Angular\cite{angular} & 512 & 54.7 & 66.3 & 76.0 & 83.9 & 61.1 \\
% HDC\cite{hdc} & 384 & 53.6 & 65.7 & 77.0 & 85.6 & - \\
% BIER\cite{bier} & 512 & 55.3 & 67.2 & 76.9 & 85.1 & - \\
% HTL\cite{htl} & 512 & 57.1 & 68.8 & 78.7 & 86.5 & - \\
% A-BIER\cite{abier} & 512 & 57.5 & 68.7 & 78.3 & 86.2 & - \\
% HTG\cite{htg} & - & 59.5 & 71.8 & 81.3 & 88.2 & - \\
% \hline
% DREML\cite{dreml} & 9216 & 63.9 & 75.0 & 83.1 & 89.7 & 67.8 \\
% \hline
% Semihard\cite{semihard} & - & 42.6 & 55.0 & 66.4 & 77.2 & 55.4 \\
% Semihard* & 128 & 56.8 & 69.1 & 79.8.7 & 87.6 & 63.0 \\
% \textbf{COD+semih} & 128 & - & - & - & - & - \\
% Margin\cite{margin}     & 128 & 63.6 & 74.4 & 83.1 & 90.0 & 69.0 \\
% Margin*                 & 128 & 62.9 & 74.1 & 82.9 & 90.0 & 66.3 \\
% \textbf{COD+margin}     & 128 & \textbf{66.6} & 76.5 & 84.8 & 90.9 & \textbf{69.0} \\
% \hline
% Semihard* & 512 & 60.6 & 72.3 & 82.3 & 88.9 & 64.5 \\
% \textbf{COD+semih} & 512 & - & - & - & - & - \\
% % \textbf{COD+margin}  & 256 & - & - & - & - & - \\
% Margin* & 512 & 65.1 & 75.6 & 84.2 & 90.7 & 67.2 \\
% \textbf{COD+margin} & 512 & - & - & - & - & - \\
% % \hline\hline
% \hline
% \end{tabular}
% \end{center}
% \label{tab:cub}
% \caption{Recall@k for k nearest neighbor and NMI on CUB200-2011 \cite{cub200-2011}. (*) indicates our best re-implementation with ResNet50.}
% \end{table}


